Exploring the Use of Abusive Generative AI Models on Civitai

The rise of generative AI is transforming the landscape of digital imagery, and exerting a significant influence on online creative communities. This has led to the emergence of AI-Generated Content (AIGC) social platforms, such as Civitai. These distinctive social platforms allow users to build and share their own generative AI models, thereby enhancing the potential for more diverse artistic expression. Designed in the vein of social networks, they also provide artists with the means to showcase their creations (generated from the models), engage in discussions, and obtain feedback, thus nurturing a sense of community. Yet, this openness also raises concerns about the abuse of such platforms, e.g., using models to disseminate deceptive deepfakes or infringe upon copyrights. To explore this, we conduct the first comprehensive empirical study of an AIGC social platform, focusing on its use for generating abusive content. As an exemplar, we construct a comprehensive dataset covering Civitai, the largest available AIGC social platform. Based on this dataset of 87K models and 2M images, we explore the characteristics of content and discuss strategies for moderation to better govern these platforms.

==> sections/old.4.RQ1.tex <==
\section{RQ1: Characterizing Users}

In this section, we characterize the users' activities. This helps us gain a deeper understanding of how the model marketplace ecosystem works and how participants interact with it.\gareth{If you wanna theme the paper around RQs, you probably wanna open each section with a question themed intro}

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.49\linewidth]{figs/rq1/following_matrix.pdf}
    \includegraphics[width=0.49\linewidth]{figs/rq1/daily_model_count.pdf}
    \caption{(a) Pairwise $R$ values (\textpertenthousand) for the 4 types of users; (b) Daily count of the uploaded models.}
    \label{fig:rq1_1}
\end{figure}

\subsection{User Types}
\label{subsec:rq1_user_type}
We begin by categorizing users into different types and assessing their significance within the ecosystem.
As discussed in \S\ref{sec:background}, Civitai has two main aspects: models and images.
Therefore, there are 4 types of users in Civitai, model-only creators (M), image-only creators (I), model-and-image creators (MI), and non-creators (N).

\gareth{It'd be good to briefly state how each of these things helps answer RQ1. You always want to ensure the reader knows how each piece of the analysis fits into the big picture}

\pb{Proportion of User Types.}
We first investigate the number of users in each type. In total, we identify 56,779 creators. Meanwhile, there are over 2 million registered users, and one does not need an account to consume content in Civitai.
\gareth{Why is it unsurprising? It is not the opposite? Why are there all these accounts, if they don't need one to consume content and they don't submit any models?}
As a result, it is unsurprising that the number of non-creators far exceeds the number of creators.
% 
We then further look into the creators. We find 4,233 (7.5\%) model-only creators, 45,147 (79.5\%) image-only creators, and 7,399 (13\%) model-and-image creators. Overall, the results indicate that the majority of users are non-creators, and among the creators, the majority are image creators.

\pb{Followers.}
The following/follower relationship among users offers another perspective on the significance of user types.
% 
Let $S_A$ be the set of users of type $A$, and $S_B$ be the set of users of type $B$. We define $F(A,B)$ as the set of pairs $(U, V)$ where $U \in S_A$ and $V \in S_B$ and $U$ follows $V$. In other words, $F(A,B)$ represents the total number of following relationships from $S_A$ to $S_B$.
% 
We then define $R(A, B)$ as $\frac{|F(A,B)|}{|S_A| \times |S_B|}$, which represents the ratio of $F(A,B)$ to the total number of possible following relationships from $S_A$ to $S_B$. In essence, $R(A, B)$ signifies the level of interest one user type shows in another. More type-$A$ users following type-$B$ users leads to greater $R(A, B)$.

Figure \ref{fig:rq1_1}a displays the pairwise $R$ values for the 4 types of users. When analyzing non-creators, only those who follow at least one other user are considered. It is clear that model-and-image creators are the most popular, then is model-only creators.  Conversely, image-only creators have much smaller $R$ values. Overall, the results indicate that, despite their smaller proportion, model creators play a significant role within the ecosystem, actively followed by all types of users.

\subsection{Model types}
The types of models that the creator uploads are also an important aspect. Figure \ref{fig:rq1_1}b shows the number of daily uploaded models. We see that the number of base models (checkpoint) remains stable (around 20) over time. Meanwhile, since it was first proposed, the number of LoRA models has risen sharply and constitutes the majority, at around 84\% of the total as of \texttt{2023-11}. LoRA (Low-rank Adaptation) models are smaller models used to fine-tune the base (checkpoint) models \cite{hu2022lora, lora-sd}. 
Note, LyCORIS \cite{yeh2024navigating} models (further extensions of LoRA) are also classified into LORA in our analysis. These are commonly used to present more specific themes, such as a specific person, clothes, art style, pose, etc., which could potentially be a source of abusive content, such as a deepfake model for a specific person. This is an important issue given the significant number and proportion of LoRA models in Civitai, which we further explore in \S\ref{sec:theme}.
\gareth{What's the takehome implication? Is there something important you can flag from this? If not, you may want to try and emphasise that this is intended to just be descriptive. }

\subsection{Content creation \& consumption}
Next, we investigate the content creation and consumption behaviors. This helps us gain a better understanding of the dynamics within the ecosystem. 

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/rq1/creation.png}
    \caption{(a) CDF of the number of creations for users; (b) The number of creations \vs the number of active days of creators.}
    \label{fig:rq1_2}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/rq1/consumption.pdf}
    \caption{(a) CDF of the download count of the model and the view count of the image; (b) Distribution of download counts for models and view counts for images.}
    \label{fig:rq1_3}
\end{figure}

\pb{Creator productivity.}
First, we analyze the productivity of creators based on the number of their creations. Figure \ref{fig:rq1_2}a displays the CDF of the number of creations per user. It is evident that model-image creators are more active compared to model-only and image-only creators. This corresponds with our earlier discovery that model-image creators are more likely to be followed. Additionally, we observe that model creators are less productive than image creators (stat \fillin). This is intuitive, as training a model is typically more difficult than generating an image.

%\pb{Active patterns.}
We then delve deeper into the active pattern of the creators. Figure \ref{fig:rq1_2}b illustrates the scatter of the number of creations \vs the number of active days of creators. It is evident that, with the same number of active days, creators are able to produce  significantly more images compared to models. On average, creators produce \fillin images per active day compared to \fillin models per active day. This suggests that image creators tend to upload a large number of images on the same day. This is mainly because they tend to upload a set of images generated by the same (or slightly tuned) prompts.



\pb{Content consumption.}
\james{Maybe we can move this part to sec~\ref{sec:reaction}, and change the name into sth like ``general overview of ...''}
We finally examine the behavior of content consumption. Figure \ref{fig:rq1_3}a illustrates the CDF of the download count of the model and the view count of the image, which indicates the level of content consumption. We see that models are more actively ``consumed'' than images (465 \vs 36 at the median), which is consistent with our findings in \S\ref{subsec:rq1_user_type} that model creators are more popular. However, it is worth noting that most images still receive some views (only 4.7\% of the images receive 0 view), with the most popular ones reaching 100k views. Considering the significantly higher number of images, they also play an important role in content consumption. \gareth{This sentence sounds a bit odd. What is the key conclusion you wanna draw here?}

Moreover, Figure \ref{fig:rq1_3}b depicts the distribution of download counts for models and view counts for images. It is evident that the top 25\% of the models and images account for 80\% of the consumption. This outcome suggests a power-law-like distribution, which is commonly observed in most user-generated-content (UGC) platforms \cite{4801529, ugander2011anatomy, 10.1145/1772690.1772751}. This also implies that content consumption behavior is centralized around a few most popular creations. We therefore want to gain a better understanding of what makes them popular, particularly regarding their themes. For example, we want to investigate whether abusive content, such as deepfake models, is more popular than other models. We further explore this in \S\ref{sec:reaction}.


\gareth{The above does not really extract any major messages. What are the key takehomes you wanna deliver here? Is there a final 'answer' to the RQ you could list here? }


% % \subsection{Primary types of models and images}

% \subsection{Creators' creative activities}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=.9\linewidth]{figs (tmp)/daily_model_count.pdf}
%     \caption{Temporal distribution of the count of created models in distinct types.}
%     \label{fig:temp_model}
% \end{figure}

% \pb{Overview of creators' productivity.} 

% \james{Distribution of distinct types of creators -- only model, only image, both? Distribution of produced model (image) per model (image) creators?}

% \pb{Temporal analysis of model creation.} To better understand the frequency of model creation on Civitai, we here perform an analysis on temporal distribution of daily shared models in distinct types. According to Figure~\ref{fig:temp_model}, \james{...}
